Statistical inference for a stochastic generalized logistic differential equation

This research aims to estimate three parameters in a stochastic generalized logistic differential equation. We assume the intrinsic growth rate and shape parameters are constant but unknown. To estimate these two parameters, we use the maximum likelihood method and establish that the estimators for these two parameters are strongly consistent. We estimate the diffusion parameter by using the quadratic variation processes. To test our results, we evaluate two data scenarios, complete and incomplete, with fixed values assigned to the three parameters. In the incomplete data scenario, we apply an Expectation Maximization algorithm.

==> intro_sdiv.tex <==
\paragraph{Logistic equation} 
The logistic growth model, an ordinary differential equation defined as 
\begin{equation}
    \label{eqn:logistic_verhulst}
    X^{\prime}(t) = 
    \alpha X(t)
    \left[
    1-\frac{X(t)}{K}
    \right],
\end{equation}
is one of the most important models in population dynamics.
Proposed by Verhulst in 1838 (see e.g.,  \cite{Vogels1975})
it remains a classic model for studying
population growth and as a cornerstone in more complex structures.
The scope of this application encompasses various fields, such as 
economics, finance, chemistry, and biology, among others. 

After Verhulst presente this model as an improvement to the Mathus 
exponential growth description
$
    X'(t) = \alpha X(t).
$
The logisitc Verhuls's model has been rediscovered and
generalized in various fields. Richards conducted in 1959 a 
well-known generalization in \cite{Rich1959}.
Richards suggested a shape parameter $m$ to
extended the Von Bertanffy growth function to fit plant data. Its generalization
rads as follows.

\begin{equation}\label{det-GLDE}
    \left.
    \begin{aligned} 
        X'(t)&= 
            \alpha X(t)
            \Bigg[
                1 - 
                \Bigg(
                    \frac{X(t)}{K}
                \Bigg) ^ m
            \Bigg],
        \quad t>t_0
        \\
        &X(t_0)= x_0,
            \quad
                x_0\in(0, K)
    \end{aligned}
    \right\}.
\end{equation}
According to \cref{det-GLDE}, if the initial population size $x_0$ 
is a positive and less than the carrying capacity $K$, then  $X(t)$ denotes 
the population size a time $t$ that grows at rate  $\alpha$ and limited by 
a finite number $K$ of natural resources.
By introducing this new parameter $m$, the logistic sigmoid shape of the 
previous model \eqref{eqn:logistic_verhulst} enchances more plasticity and 
expands its fitting range. For values of $m$ in $(0,1)$, the sigmoid 
function tends towards a linear activation function, while for $m>1$, the 
sigmoid shape becomes similar to the Heaviside step function. Moreover, 
according to \cite{Rich1959}, this generalization encompasses different 
values of $m$, which accounts for well-known growth modes such as the 
monomolecular, auto-catalytic, and Gompertz. 

Certain studies suggest that the logistic Richards' model yields more 
precise results when fitting real data. For instance, Qin et al. observed 
better performance with the Richards' model \eqref{det-GLDE} than with the 
Verhulst model \cref{eqn:logistic_verhulst} when calibrating a database of 
monthly smoothed international sunspot number \cite{Qin2018}.

\Cref{det-GLDE} is a particular instance of the Bernoulli differential 
equation. When we substitute $u$ by $X^{1-m}$ in \cref{det-GLDE}, 
it becomes a linear equation that we can solve using an integral factor.
This argument leads us to the following solution
\begin{equation}
    X(t)
        =\frac{K}{(1+Q e^{-\alpha m (t-t_0)})^{1/m}},
    \qquad  
    Q:=
    \left(
    \frac{K}{x_0}
    \right)^m - 1.
\end{equation}

Assuming this model represents biological growth, we can fix parameter $K$ using 
prior biological experience or consider it the maximum value of actual 
observations. So, we can resacalete the dynamics of eqution in termis of this 
parameter. When we rescale equation (2) in terms of the carrying capacity $K$, we 
get dynamics that fall within the interval $(0,1)$, with two fixed points at 
$X^{\star}=0$ and $X^{\star \star}=1$. The point $X^{\star}$ is unstable, while 
the point $X^{\star \star}$ is asymptotically stable for any initial condition 
$x_0 \in (0,1)$.


\paragraph{Stochastic extension}

When analyzing data from natural sources, it is essential to account for 
uncertainty in practical applications. As a result, recent research on population 
growth has extended \Cref{det-GLDE} to include uncertinity. 
For further reading, we recommend checking out the works \cite{Cortes2019}, 
\cite{Schurz2007}, \cite{su} among others.

In this paper, we address the parametrization of a stochastic extension of the 
generalized logistic equation described in \eqref{det-GLDE}, namely: 
\begin{equation}
    \label{SGLDE}
    \left.
    \begin{aligned}
        dX(t) &= 
        \alpha X(t)
        \left(
            1 - X(t) ^ m
        \right)
        dt
         +
        \sigma X(t) dB(t),
        \  t>t_0,
        \\
        X(t_0)&= x_0
    \end{aligned}
    \right\}.
\end{equation}
%
Here, $x_0 \in (0, 1)$, and $\{B(t)\}_{t\geq t_0}$ 
is a standard Brownian motion and the solution process $X(t, \omega)$ 
is understood under the usual conditions. That is, we assume that
solution $X$ and $x_0$ are defined on a common filtrated 
probability space 
$
    (
        \Pb, 
        \Omega,
        \cf
    )
$, with filtration $\cf =\{ \cf \}_{t\geq 0}$ generated by the Brownian process
$B(t)$. \Cref{SGLDE} is a Itô-stochastic differential equation (SDE) driven by a
multiplicative noise. 

Using It\^o's formula we obtain the closed solution to \eqref{SGLDE}
(see \cite{su} for further reading) 

\begin{equation}
    \label{sol-SGLDE}
    \begin{aligned}
        X(t) = x_0 \,& 
        \exp
        \Big[  
            \Big(
                \alpha - \frac{1}{2}\sigma^2
            \Big) t 
            + 
            \sigma B(t)
        \Big]
        \\
        &\, 
        \times 
        \Bigg[
            1 +  
            x_0 ^ m
            \alpha m 
            \int_0^t 
                \exp
                    \Big[
                        \Big(
                            \alpha - \frac{1}{2} \sigma^2
                        \Big) s
                        + \sigma B(s)
                    \Big]  ds 
        \Bigg] ^ {-1/m}.
    \end{aligned}    
\end{equation}
We observe that the solution is always positive for all $t\ge 0$.
From the above we can prove that
$$
\lim_{t\rightarrow\infty}  \E [X(t)]= 1,
$$
\paragraph{Aim}
We assume that the parameters $\alpha, m$, and $\sigma$ are 
constants but unknown.  In this manner, we aim for two main objectives.
The former is to develop a framework based on the so-called Estimation 
Maximization (EM) algorithm [CITE] to estimate parameters $\alpha,m$, and 
$\sigma$. The latter is extended to these estimators to deal with incomplete 
information.

\paragraph{Literature Review}
Several contributions have reported formulations that are 
closely related to the model presented in equation \eqref{SGLDE}. However, 
to the best of our knowledge, only \cite{Bevia2023}provides details on 
parameter calibration using real  data, but with a model based on a random 
differentialequation. Suryawan \cite{su} evaluates some qualitative aspects 
of the solution, such as long-time behavior and noise-induced transition, 
using the framework of Ito's stochastic calculus. Cortes et al. 
\cite{Cortes2019} obtain the probability density of the underlying solution 
processes using the Karhunen–Lo\`{e}ve expansion and other transformations. 
Most of the literature focuses on the  model \eqref{SGLDE} with $m=1$. Other 
authors such as \cite{Liu2013, Braumann2008} document the qualitative 
behavior of the solution process using a different form of diffusion term. 
Nevertheless, \cite{Schurz2007} 
presents a theory and exhaustive numerical analysis for other linear 
generalizations in the drift and nonlinear terms in the diffusion term.

%\paragraph{Contribution}
\paragraph{Overview}
